DE-HNN: An effective neural model for Circuit Netlist representation

The run-time for optimization tools used in chip design has grown with the complexity of designs to the point where it can take several days to go through one design cycle which has become a bottleneck. Designers want fast tools that can quickly give feedback on a design. Using the input and output data of the tools from past designs, one can attempt to build a machine learning model that predicts the outcome of a design in significantly shorter time than running the tool. The accuracy of such models is affected by the representation of the design data, which is usually a netlist that describes the elements of the digital circuit and how they are connected. Graph representations for the netlist together with graph neural networks have been investigated for such models. However, the characteristics of netlists pose several challenges for existing graph learning frameworks, due to the large number of nodes and the importance of long-range interactions between nodes. To address these challenges, we represent the netlist as a directed hypergraph and propose a Directional Equivariant Hypergraph Neural Network (DE-HNN) for the effective learning of (directed) hypergraphs. Theoretically, we show that our DE-HNN can universally approximate any node or hyperedge based function that satisfies certain permutation equivariant and invariant properties natural for directed hypergraphs. We compare the proposed DE-HNN with several State-of-the-art (SOTA) machine learning models for (hyper)graphs and netlists, and show that the DE-HNN significantly outperforms them in predicting the outcome of optimized place-and-route tools directly from the input netlists. Our source code and the netlists data used are publicly available at https://github.com/YusuLab/chips.git

==> Supplement_lastmin.tex <==
\aistatstitle{Supplement of the AISTATS submission \#1797, \\Title: ``DE-HNN: An effective neural model for Circuit Netlist representation"}

\section{More Background}
\label{appendix:background}

\subsection{Circuit netlists}
A circuit netlist is a textual representation of electronic components, such as logical boolean gates, and the connections between them. Figure 1 provides an example illustrating a circuit netlist consisting of five components interconnected by five nets. After laying out the netlist in the physical space (placement), during the routing stage, the edges of the netlist are mapped to the routing channels within the chip's physical floorplan (indicated by dashed lines in Figure \ref{fig:circuit_diagram}). Routing congestion occurs when the number of edges to be routed in a specific region of the floorplan exceeds the available routing capacity.
\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.4]{figures/circuit_diagram.jpeg}
    \caption{Visulization of a circuit netlits in the {\bf post place-and-route} stage: Each cell ($C_i$) is positioned within the physical layout of the chip and interconnected with other components following the net maps ($\sigma_i$).}
    \label{fig:circuit_diagram}
\end{figure}

\subsection{Persistence homology based features}
\label{appendix:PD}

Persistent homology is one of the most important development in the field of topological data analysis in the past two decades. It can encode meaningful topological features in a multi-scale manner and has already been applied to numerous applications; see books \citep{EH10, DW22}. 
Intuitively, given a domain $X$, a $p$-th homology class (or informally, a $p$-th homological feature) essentially captures a family of equivalent $p$-dimensional ``holes'' in $X$; for example, 0-, 1- and 2-dimensional homology captures connected components, equivalent classes of loops and of 2-dimensional voids, respectively. The $p$-th homology group $\mathrm{H}_p(X)$ (using $\mathbb{Z}_2$ coefficients) characterizes the space of $p$-th homological features of $X$, and its rank $rank(\mathrm{H}_p(X))$ corresponds to the number of independent $p$-th homological features. For example, $rank(\mathrm{H}_0(X))$ denotes the number of connected components of space $X$. If the domain $X$ is a graph, then its $1$-st homology group is homeomorphic the space of cycles (loops), and $rank(\mathrm{H}_1(X))$ is simply the number of independent cycles. 

Persistent homology is a modern extension of homology, where instead of a single space $X$, we now inspect a sequence of growing spaces $X_1 \subseteq X_2 \subseteq \cdots X_m = X$, called a \emph{filtration} \footnote{Note that persistent homology has been extended for much broader families of filtrations then the growing sequence we describe here; see \citep{EH10, DW22}.}. Intuitively, we can view this filtration as an evolution of the space $X$. As the space grows, we track its corresponding topological features (as captured by the homology groups introduced above). Sometimes new topological features (e.g., a new component, or a hole) will appear, and sometimes they will disappear (e.g, a hole is filled and thus ``disappear''). The \emph{persistent homology (PH)} captures such creation and death of topological features, and outputs a feature summary called \emph{persistent diagram (PD)}, consisting of the birth-time and death-time of classes of topological features during this evolution. In short, the PDs provide a multiscale summary for the topological features of $X$ from the perspective of filtration $X_1\subseteq X_2\subseteq \cdots \subseteq X_m$. In the past few years, there have been a series of approaches to vectorize PDs or to kernelize them for ML applications; see Chapter 13 of \citep{DW22}. In our work, we use the so-called \emph{persistence images} \citep{JMLR:v18:16-337} to convert a PD to a finite dimensional vector to be used as part of the node feature. 

\paragraph{Persistence diagram (PD) induced from Netlists.}
We compute the persistence diagram (PD) based on the following directed graph representation of the netlist (instead of using the directed hypergraph representation, for easier computation of persistence). 

In particular, given a netlist, we create a directed graph $G = (V, E)$ where each node in $V$ correspoinds to a cell in the netlist, while a directed edge is formed between the driver cell of some net with each of the sink in that net; that is, each net $\sigma = (\dr_\sigma, \sinkset_\sigma)$ gives rise to a set of directed edges $\{(\dr_\sigma, v)\}_{v\in \sinkset_\sigma}$. 
We refer to this graph as the \emph{star-graph} induced by the input netlist. 

Now, for each node $v$ in the star-graph $G$, we create its $k$-ring \emph{out-flow neighborhood $G^{in}_v$} which is simply the subgraph in $G$ spanned by all nodes reachable from $v$ by a path of at most $k$ hops. 
Symmetrically, the $k$-ring \emph{in-flow neighborhood $G^{out}_v$} of $v$ is the subgraph of $G$ spanned by all nodes such that $v$ is reachable within $k$ hops. These two $G_v$s form the \emph{local motifs} around $v$.
We wish to obtain a feature vector summary for $G^{in}_v$ and $G^{out}_v$. 
To this end, similar to \citep{yan2021link,zhao2020persistence}, we use the so-called \emph{$0$th extended persistence diagram} $PD^{*}_v$ \citep{cohen2009extending} of $G^*_v$ (where $* \in \{in, out\}$) induced by the shortest path distance function to $v$ as its summary. 
For our specific graph settig, using results of \citep{TW19}, one can show that $PD^*_v$ computed this way, is a concise summary that encodes rich information around $v$, including the number of triangles incident to $v$, clustering coefficient of $v$, number of nodes at distance $r \le k$ away from $v$, number of crossing edges from distance-$r$ nodes to distance ($r+1$) nodes, certain ``shortest" system of cycle basis passing through $v$ of $G^*_v$, and so on. 
Finally, each PD (for in-flow neighborhood and out-flow neighborhood of $v$) is vectorized to persistent images as in \citep{JMLR:v18:16-337}, and we further vectorize (flatten) each image matrix all together to generate a new vector as the persistent representation vector for each node. 

\section{Theoretical Analysis} \label{sec:theoretical_analysis}
\subsection{Preliminaries}\label{sec:prelim}
Let $\mathbb{D}$ be a domain, namely, $\mathbb{Q}, \mathbb{R}$, and $\mathbb{R}^d$. Consider the set function $f : 2^{\mathbb{D}} \rightarrow \mathrm{codom}(f)$ where $\mathrm{D}$ is a countable domain. Then, we have 
\[
    \forall X \subseteq \mathbb{D}: f(X) = \rho \circ \Phi(X), \ \ \Phi(X) = \sum_{x \in X} \phi(x),
\]
where $\phi:\mathbb{D} \rightarrow \mathbb{R}$, and $\rho: \mathbb{R} \rightarrow \mathrm{codom}(f)$. This is the sum-decomposable representation of $f$ via $\mathbb{R}$ in terms of $(\phi, \rho)$ basis functions. We refer to $\mathrm{codom}(\phi)$ the model’s latent space~\citep{NIPS2017_f22e4747}. There is an extended sum-decomposable representation of $f$ on multi-sets whose elements are drawn from an uncountable domain (e.g., $\mathbb{R}$) by restricting the size of input multi-sets. For any domain $\mathrm{D} \subseteq \mathbb{R}^d$, denote the set of sub-multi-sets of $\mathbb{D}$ that contain at most $N$ elements by $\mathbb{D}^{\leq N}$. 
\begin{theorem}[\citep{wagstaff2019limitations}]
    Let $N \in \mathbb{N}$, and $f : [0, 1]^{\leq N} \rightarrow \mathbb{R}$ be a continuous set function.
    Then, it is continuously sum-decomposable via $\mathbb{R}^{N}$ --- that is, $\rho$ and $\phi$ are continuous functions and the latent space is a subset of $\mathbb{R}^{N}$  --- and vice versa.\label{thm:continuously_sum_decomposable_1d}
\end{theorem}
\Cref{thm:continuously_sum_decomposable_1d} provides universal representation of multi-set functions over inputs with scalar elements. If we fix the size of the inputs, multi-set functions become equivalent to permutation-invariant functions. We can universally approximate continuous permutation-invariant functions over a compact set of multivariate elements with a permutation-invariant polynomial. Permutation-invariant polynomials have $K = {N+d \choose d}-1$ power-sum multi-symmetric polynomials basis~\citep{rydh2007minimal}, i.e.,
\[
    \forall X \in \mathbb{X}_{N,\mathbb{R}^d} : \ p(X) = \mathrm{poly}(e_1(X), \cdots,e_K(X)),
\]
where $e_k(X)=\sum_{x \in X} \prod_{i=1}^d x_{i}^{k_i}$ is a power-sum multi-symmetric polynomial, $k_1 \ldots k_d$ is the $d$-digit representation of $k \in [K]$ in base $N+1$, $K = {N+d \choose d}-1$, $\mathrm{poly}$ is a polynomial function~\citep{rydh2007minimal}, and $\mathbb{X}_{N,\mathbb{R}^d} = \{ \{ \{ x_n \} \}_{n = 1}^{N}: x_n \in \mathbb{R}^d \ \forall n \in [N] \}$, that is, the set of multi-sets of size $N$ drawn from $\mathbb{R}^d$. This is at core of the existing universal approximation results for continuous permutation-invariant functions over multivariate elements via $\mathbb{R}^{K}$~\citep{NIPS2017_f22e4747,maron2019provably,segol2019universal}. 
That is, we can design an encoder $\phi$ that maps to $\mathbb{R}^K$ and provides a universally approximate sum-decomposable model for continuous multivariate permutation-invariant functions; see Theorem 9 in \citep{NIPS2017_f22e4747} and \citep{maron2019provably,segol2019universal}. Recently, Fereydounian \emph{et al.}~\citep{fereydounian2022exact} proposed a novel encoding function $\phi: \mathbb{R}^d \rightarrow \mathbb{R}^{O(d^2) \times N}$ such that $\Phi(X) = \sum_{x \in X} \phi(x)$ is an injective map whose inverse is continuous, that is, $\Phi^{-1} \circ \Phi(X) = X$ --- a significant reduction in the latent dimension for universal representation when $d \geq 2$, i.e.,
\[
    \forall X \in \mathbb{X}_{N,\mathbb{R}^d} : f(X) = \rho \circ \Phi(X),
\]
where $\rho = f \circ \Phi^{-1}$ is a continuous function over its domain. At their core, sum-decomposable models rely on a bijection between multi-sets and encoded features, that is, $X = \alpha \circ \Phi(X)$ for any multi-set $X \in \mathbb{X}_{N,\mathbb{R}^d}$ and a bijective map $\alpha$. In the following proposition, we first generalize this result to multi-sets with variable sizes.
\begin{proposition} \label{prop:multivariate_continuous_bijection}
   Let $\mathcal{B}$ be a connected compact subset of $\mathbb{R}^d$. There exists a function $\phi: \mathbb{R}^d \rightarrow \mathbb{R}^{d^{\prime}}$ such that 
    \[
        \forall X \in \mathbb{X}_{\leq N, \mathcal{B}}: X = \alpha \bigg( \sum_{x \in X} \phi(x) \bigg)
    \]
    where $\mathbb{X}_{\leq N, \mathcal{B}}$ is all multi-sets of size $\leq N$ with elements from $\mathcal{B}$, $\alpha$ is a continuous map {\bf over its domain} and $d^{\prime}$ depends on $N$ and $d$.
\end{proposition} 

\begin{proof}
\citet{fereydounian2022exact} proposed a novel encoding function $\phi: \mathbb{R}^d \rightarrow \mathbb{R}^{ O(d^2) \times N}$ such that $\Phi(x) = \sum_{x \in X} \phi(x)$ is an injective map over multi-sets with exactly $N$ elements, that is, $\Phi^{-1} \circ \Phi(X) = X$ where elements of multi-set $X$ is drawn from $\mathbb{R}^d$ and $|X| = N$. Moreover, the inverse function $\Phi^{-1}$ is continuous over $\mathrm{codom}(\Phi) = \{ \Phi(X): X \in \mathbb{X}_{N, \mathcal{B}}\}$ where $\mathcal{B}$ is a compact and connected subset of $\mathbb{R}^d$. To extend their result to multi-sets of variable sizes, we follow the proof sketch for the one-dimensional case \citep{wagstaff2019limitations}. Let $x_{\circ} \in \mathbb{R}^{d} \setminus \mathcal{B}$. Then, we define $\phi^{\prime}(x) = \phi(x) - \phi(x_{\circ})$. For any multi-set with $M \leq N$ elements from $\mathcal{B}$, say $X$, we have
    \begin{align*}
        \forall X \in \mathbb{X}_{\leq N, \mathcal{B}}: \Phi^{\prime}(X) &= \sum_{x \in X} \phi^{\prime}(x) = \sum_{x \in X}  \phi(x) - M \phi(x_{\circ} ) \\
        &= \Phi( X \cup \{ \{ \underbrace{x_{\circ} , \ldots, x_{\circ} }_{N-M} \} \} ) - N \phi(x_{\circ} ) \\
        &= \Phi( X \cup \{ \{ \underbrace{x_{\circ} , \ldots, x_{\circ} }_{N-M} \} \} )+\mathrm{const},
    \end{align*}
where $\mathrm{const} = -N \phi(x_\circ) $ and $\mathbb{X}_{\leq N, \mathcal{B}} = \bigcup_{n = 1}^{N} \mathbb{X}_{n, \mathcal{B}} $. This is in the sum-decomposable form. Since $\Phi$ is an injective map over $\mathbb{X}_{N, \mathcal{B}}$, $\Phi^{\prime}$ is also an injective map. That is, we have
    \begin{align*}
         \Big( \Phi^{-1} \circ (\Phi^{\prime} (X)  - \mathrm{const} \big) \Big) \cap \mathcal{B}  &= \Big( \Phi^{-1} \circ  \Phi ( X \cup \{ \{ \underbrace{x_{\circ} , \ldots, x_{\circ} }_{N-M} \} \} )  \Big) \cap \mathcal{B}   \\
         &= ( X \cup \{ \{ \underbrace{x_{\circ} , \ldots, x_{\circ} }_{N-M} \} \} )  \cap \mathcal{B} \\
         &= X,
    \end{align*}
that is, ${\Phi^{\prime}}^{-1}(U) = \Phi^{-1} \big( U  - \mathrm{const} \big) \cap \mathcal{B}$ for all $U \in \mathrm{codom}(\Phi^{\prime}) = \{ \Phi^{\prime}(X): X \in \mathbb{X}_{\leq N, \mathcal{B}} \}$.

Let us now show that ${\Phi^{\prime}}^{-1}$ is a continuous map over $\mathrm{codom}(\Phi^{\prime})$. We have to show that for all $\varepsilon >0$ such that $d( {\Phi^{\prime}}^{-1} \circ \Phi^{\prime}(X) ,  {\Phi^{\prime}}^{-1} \circ \Phi^{\prime}(Y) ) < \varepsilon$, there exists a $\delta >0$ such that $\| \Phi^{\prime}(X) - \Phi^{\prime}(Y)\|_2 < \delta$ where $X, Y \in \mathbb{X}_{\leq N, \mathcal{B}}$ and $d$ is the matching distance between multi-sets, i.e.,
\[
    d(X, Y) = \begin{cases}
        \min_{ \text{bijection} \ \pi : X \rightarrow Y } \sqrt{\sum_{x \in X} \| x -\pi(x) \|_2^2} & \mbox{if} \ \ |X| = | Y | \\
        \infty & \mbox{if}  \ \ |X| \neq | Y |.
    \end{cases} 
\]
Let us pick $\varepsilon > 0$. If $d( {\Phi^{\prime}}^{-1} \circ \Phi^{\prime}(X) , {\Phi^{\prime}}^{-1} \circ \Phi^{\prime}(Y) ) < \varepsilon$, then we must have $|X| = |Y|$, that is, $X$ and $Y$ have the same sizes. Therefore, we have
\[
    d( {\Phi^{\prime}}^{-1} \circ \Phi^{\prime}(X) -  {\Phi^{\prime}}^{-1} \circ \Phi^{\prime}(Y) ) = d( X , Y) < \varepsilon.
\]
Since $\Phi^{\prime}$ is a continuous function, we conclude that $\| \Phi^{\prime}(X) - \Phi^{\prime}(Y)\|_2 < \delta$ for a $\delta >0$ that diminishes to zero as $\varepsilon \rightarrow 0$. Therefore, $(\Phi^{\prime})^{-1}$ is a continuous function over $\mathrm{codom}(\Phi^{\prime})$. If we let $\alpha = {\Phi^{\prime}}^{-1}$ and rename $\phi^{\prime}$ to $\phi$, we arrive at the proposition's statement.
\end{proof}
\subsection{Towards \Cref{thm:nested_permutation_invariant}}
We now provide some theoretical guarantee of our proposed model. We denote a directional hyperedge as $\ahyperE = (\dr_\ahyperE, \sinkset_\ahyperE )$ where $\dr_\ahyperE$ is the source node and $\sinkset_\ahyperE$ is the set of sink nodes. Considering a fixed layer $\ell$, recall that we compute features on nets via features from those cells it contains: 
\[
M^{\ell}(\ahyperE) =  \mathrm{Agg}^\ell_{v \rightarrow \ahyperE}( m^\ell(\dr_\sigma), \msetL m^\ell(v^{\prime})\msetR_{v^{\prime} \in \sinkset_\ahyperE} ). 
\]
where $\mathrm{Agg}_{v \rightarrow \ahyperE}$ is invariant to permutation of cells in $\sinkset_\ahyperE$. The general way to compute the feature of a node depends on features of the set of those nets containing it: 
\[
m^{\ell}(v) =  \mathrm{Agg}^\ell_{\ahyperE \rightarrow v} ( \msetL M^{\ell - 1}(\sigma^{\prime} )\msetR_{\sigma^{\prime} \in \NN(v)} ),
\]
where the function $\mathrm{Agg}_{\ahyperE \rightarrow v}$ is \emph{permutation invariant} to the order of neighboring nets of $v$ in $\NN(v)$. For simplicity, we assume that the input and output net features are both of the same dimension $d$ (i.e, both are from compact set $\mathcal{B}\subset \mathbb{R}^d$). The general net-value function is nested-permutation invariant and take the form of Eqn \ref{eq:M}. In what follows, we provide the detailed version of Theorem \ref{thm:nested_permutation_invariant} and show that such nested-permutation invariant function adapts a nested sum-decomposition aligned with our \DEHNN's node and net update rules. 







    

\begin{theorem}
    Let $\Fcal$ be any continuous, nested-permutation invariant, net-value function as in Eqn (\ref{eq:M}). For simplicity, assume both input nets and output of $M$ take values in a compact set $\mathcal{B} \subset \mathbb{R}^d$, 
    a connected compact subset of $\mathbb{R}^d$. We also let $N_v  = \max \{ | \NN(v )|:\forall v  \}$ and  $N_{\ahyperE} = \max \{ |\sinkset(\ahyperE)| : \forall \ahyperE  \} $.  
    Then we have that $\Fcal$ can be rewritten as the following sum-decomposition 
    \begin{align*}
     \forall \sigma: \Fcal\Big( \{ \mu_{\anet'} \}_{\anet' \in \NN(\dr_\ahyperE)} , 
\Big\{ \{  \mu_{\anet'} \}_{\anet' \in \NN(v^{\prime})}  \Big\}_{v^{\prime} \in \sinkset_\ahyperE}  \Big) = \rho \Big( \sum_{ \sigma^{\prime} \in \NN(\dr_\ahyperE) } \phi_1 (\mu_{\sigma^{\prime}}),
        \sum_{v^{\prime} \in \sinkset_\ahyperE}\phi_2\big( \sum_{ \sigma^{\prime} \in \NN(v^{\prime}) } \phi_1 (\mu_{\sigma^{\prime}}) \big) \Big),
    \end{align*} 
    where $\phi_1: \mathbb{R}^d \rightarrow \mathrm{codom}(\phi_1) \subseteq \mathbb{R}^{d^{\prime}(d,N_v)}$, $\phi_2: \mathbb{R}^{d^{\prime}(d,N_v)} \rightarrow \mathrm{codom}(\phi_2) \subseteq \mathbb{R}^{d^{\prime \prime}(d,N_v,N_{\ahyperE})}$, and $\rho$ are continuous functions on their domains.
\end{theorem} 



\begin{proof}
The general net-value function takes the following form:
\begin{align*}
    \forall \sigma: ~& \Fcal\Big( \{ \mu_{\anet'} \}_{\anet' \in \NN(\dr_\ahyperE)} , 
\Big\{ \{  \mu_{\anet'} \}_{\anet' \in \NN(v^{\prime})}  \Big\}_{v^{\prime} \in \sinkset_\ahyperE}  \Big) \nonumber.
\end{align*}
We assume $\Fcal$ is a continuous function that takes values in $\mathcal{B}$, a connected compact subset of $\mathbb{R}^d$, and $N_v  = \max \{ | \mathcal{N}(v)|:\forall v  \}$. 

Since $\mathcal{F}$ is a contiuous function that is permutation invariant and polynomials universal approximators, then there exist continuous functions $\phi_1$ and $\alpha_1$ 

\begin{align*}
    \forall \ahyperE:  \mathcal{F}^{(1)} \Big(   \sum_{\sigma^{\prime} \in \NN(\dr_\ahyperE)} \phi_1 (\mu_\sigma^{\prime}) , 
    \Big\{ \{  \mu_{\anet'} \}_{\anet' \in \NN(v^{\prime})}  \Big\}_{v^{\prime} \in \sinkset_\ahyperE} 
    \Big) =  \mathcal{F}^{(1)} \Big(  \sum_{\sigma^{\prime} \in \NN(\dr_\ahyperE)} \phi_1 (\mu_\sigma^{\prime}), 
    \Big\{  \sum_{\sigma^{\prime} \in \NN(v^{\prime})} \phi_1 (\sigma^{\prime}) \Big\}_{v^{\prime} \in \sinkset_\ahyperE}  \Big)
\end{align*}
where $\mathcal{F}_1(x, Y) \stackrel{\mathrm{def.}}{=} \mathcal{F}(\alpha_1(x) , \{ \alpha_1(y) \}_{y \in Y})$ for all $x \in \mathrm{codom}(\Phi_1) = \{ \Phi_1(Y) = \sum_{y \in Y} \phi_1(y) : Y \in \mathbb{X}_{\leq N_v, \mathcal{B}} \}$  and any set $Z$ with elements in $\mathrm{codom}(\Phi_1)$. Since both $\alpha_1$ and $\mathcal{F}$ are continuous functions, then $\mathcal{F}_1$ is also continuous over its domain.



where $\mathrm{codom}(\phi_1) \subseteq \mathbb{R}^{d^{\prime}(d, N_v)}$, that is, the latent dimension depends on $d$ and $N_v$. Therefore, we apply the result in Proposition \ref{prop:multivariate_continuous_bijection} to sets of net values (of size at most $N_v$) and express $\Fcal$ follows:

Again, we can apply the result of Proposition \ref{prop:multivariate_continuous_bijection} to $\mathcal{F}_1$. The elements of the set $\Big\{ \sum_{\sigma^{\prime} \in \NN(v^{\prime})} \phi_1 (\sigma^{\prime})  \Big\}_{v^{\prime} \in \sinkset_\ahyperE}$ take values in $\mathrm{codom}(\Phi_1)$ ---  a connected compact subset of $\mathbb{R}^{d^{\prime}(d, N_v)}$. If we assume $|\sinkset_\ahyperE| \leq N_{\ahyperE}$ for all $\ahyperE$, Proposition \ref{prop:multivariate_continuous_bijection} claims that there exist continuous functions $\alpha_2$ and $\phi_2$ such that the following holds true:
\begin{align*}
    \forall \ahyperE: \mathcal{F}_1 \Big(  \sum_{\sigma^{\prime} \in \NN(\dr_\ahyperE)} \phi_1 (\mu_\sigma^{\prime}), 
    \Big\{  \sum_{\sigma^{\prime} \in \NN(v^{\prime})} \phi_1 (\sigma^{\prime}) \Big\}_{v^{\prime} \in \sinkset_\ahyperE}  \Big)
    &= \mathcal{F}_1 \Bigg(  \sum_{\sigma^{\prime} \in \NN(\dr_\ahyperE)} \phi_1 (\mu_\sigma^{\prime}), 
    \alpha_2 \Big( \sum_{v^{\prime} \in \sinkset_\ahyperE} \phi_2 \big(   \sum_{\sigma^{\prime} \in \NN(v^{\prime})} \phi_1 (\sigma^{\prime}) \big)   \Big) \Bigg) \\
    &= \rho \Bigg(  \sum_{\sigma^{\prime} \in \NN(\dr_\ahyperE)} \phi_1 (\mu_\sigma^{\prime}), 
     \sum_{v^{\prime} \in \sinkset_\ahyperE} \phi_2 \big(   \sum_{\sigma^{\prime} \in \NN(v^{\prime})} \phi_1 (\sigma^{\prime}) \big)    \Bigg)
\end{align*}
where  $\rho(x, y) \stackrel{\text{def}}{=} \mathcal{F}_1(x , \alpha_2(y) )$ for all $x \in \mathrm{codom}(\Phi_1)$ and $y \in \mathrm{codom}(\Phi_2) \stackrel{\text{def}}{=}   \{ \sum_{z \in Z}\phi_2(z): Z \in \mathrm{codom}(\Phi_1), |Z| \leq N_{\ahyperE} \} $. The function $\rho$ is a composition of continuous functions $\mathcal{F}_1$ and $\alpha_2$. Therefore, it is continuous on its domain. Finally, the dimension of the codomain of $\phi_2$ is a function of $d^{\prime}(d, N_v)$ and $N_{\ahyperE}$, that is, $d^{\prime \prime}(d, N_v, N_\ahyperE)$.
\end{proof}



\section{Experimental details}

\subsection{Dataset Statistics}
\label{appendix:statistics}

We report the sizes of each design and their cell/net-degrees distribution in Table~\ref{table:dataset}, and net-based demand/wirelength distributions in the Table~\ref{table:distribution}. We can see that (hyper)graphs in our dataset are large and sparse, ranging from 400K to 1.4M nodes. 
with few outliers that have high degrees. We also summarize the more detailed distributions of net-based demand, net-based wirelength, and cell-based congestion in figure\ref{fig:statistics_hist}. 

\subsection{Experiment Setup}
\label{appendix:setup}

We engineer the input features as Cell features and Net features. None of the following features contained placement information or are computed from placement information. We engineer cell features as follows:
\begin{itemize}
\item We analyze the statistics in a design including the minimum and maximum of all cells' width, height. Then, we normalize all these quantities to be in the range $[0, 1]$. We concatenate them with the cell's discrete orientation and cell's degree (number of nets each cell connecting to), that results into the cell's input feature 
vector.
\item We calculate the top-10 eigenvectors of the graph Laplacian of the heterogenous graph as the positional encoding (denoted as LapPE) for every cell and net.
\item We compute the persistence diagram (denoted as PD) for each cell-node $v$ on a directed graph $G = (V, E)$, as we mentioned earlier in \ref{appendix:PD}, as a common cell-node input feature vector for all baselines, to capture the local topological information. 
\item We also compute the degree distribution for each cell-node $v$ based on their $k$-ring \textbf{\emph{undirected}} \emph{neighborhood $G_v$} in the star-graph we introduced in \ref{appendix:PD} to compute the persistence diagrams. However, we ignore the direction when we compute the degree distribution. 

\end{itemize}
For the net features, for all models other than linear Transformer, we initialize the features of each {\bf net} $\ahyperE = (\dr_\ahyperE, \sinkset_\ahyperE)$ as the net's degree (i.e.~number of cells each net connecting to). 
For Linear Transformer, in order to provide better topology information, we instead initialize the features of each {\bf net} $\ahyperE = (\dr_\ahyperE, \sinkset_\ahyperE)$ (denoted as $M(\ahyperE)$) as the average of all the features of the nodes this net contains, computed as, 
\begin{equation}\label{eq:lin_net}
M(\ahyperE) = \frac{1}{|\sinkset_\ahyperE| + 1} ( m(\dr_\sigma) +  \sum_{v^\prime \in \sinkset_\ahyperE} m(v^\prime) ). 
\end{equation}

As also described in the main text, for GCN and GATv2, we use the bipartite graph representation of the input netlist, where there are two types of graph nodes: those corresponding to cells and those corresponding nets. If a cell is contained in a net, then there is an edge between their respective graph nodes. We use {\bf heterogenous} message passing, where nodes corresponding to cells use a different message passing mechanism from nodes corresponding to nets. 

For GCN, GATv2 and HyperConv, we used 4 layers with 64 dimmensions each layer as the setting. For Linear Transformer, we used 2 layers with 64 dimmensions each layer as the setting. For NetlistGNN we used 4 layers with node dimmensions 64 and net dimmensions 64 as the setting. For All E-HNN/DE-HNN based models, we used 3 layers with node dimmensions 64. 

We report the number of parameters, training time per epoch and total training epochs in the Table \ref{table:params}. For fair comparison, note that all models have similar numbers of parameters. Interestingly, while they all take similar number of epochs to converge, our \DEHNN{} in fact is much faster per epoch, so overall takes less time to train.
We used two NVIDIA A100-SXM4-80GB GPUs on Linux CentOS Stream system (Ver.8) for both single-design and cross-design experiments. \par

\input{tables/parameters}
\input{tables/dataset_table}
\input{tables/distribution}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.90\textwidth]{figures/wirelength_distribution.pdf}
\includegraphics[width=0.90\textwidth]{figures/demand_distribution.pdf}
\includegraphics[width=0.90\textwidth]{figures/congestion_distribution.pdf}
\caption{{\small Net-based wirelength, net-based demand and cell-based congestion distributions of each design}}
\label{fig:statistics_hist}
\end{figure}

\subsection{More experimental results}
\label{appendix:results}



\input{tables/ablation_table}

\input{tables/ablation_table_pd}

In the main text, we have reported plots for ablation studies of different strategies used in our model. Here in Table \ref{table:ab} we report detailed numbers for all three tasks: net-based wirelength regression, net-based demand regression, and cell-based congestion classification across all the designs. 

Besides ablation study over our models, as we mentioned in main paper, adding the  persistence diagrams (PDs) features are beneficial for both our method and baselines. We have already shown the benefits for our model in the ablation studies in the main text and above. Here in Table \ref{table:pd-ab}, we show its benefits to the three best performing baseline models: NetlistGNN, GCN, GATv2. As we can see, using PDs improve all these models. Note that in the main text, when we report results of these baseline models, we are already reporting results with PDs. 

Finally, we show more detailed experimental results of single-design experiments for net-based wirelength regression in Table \ref{table:single-design-hpwl-full}, net-based regression in Table \ref{table:single-design-demand-full} and cell-based congestion classification in Table \ref{table:single-design-classify-full} for each design. Similar to how we report the results in the main paper, we highlight the models' results with the best performance in red, and highlight the models (other than our models) that with second best performance as blue. 
In the cases that a baseline model is better than our model, we highlight that baseline model's results in red instead. 

\input{tables/single_design_hpwl_full}
\input{tables/single_design_demand_full}
\input{tables/single_design_classify_full}



==> checklist.tex <==
\section*{Checklist}

 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [No] (We will make them public available in github together with publication of paper. )
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [No] (We will make them public available in github together with publication of paper. )
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Yes] 
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Yes]
   \item The license information of the assets, if applicable. [Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [No] (We will make them public available in github together with publication of paper.) 
   \item Information about consent from data providers/curators. [Yes]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}


 

